Provably Safeguarding a Classifier from OOD and Adversarial Samples: an Extreme Value Theory Approach

This paper introduces a novel method, Sample-efficient Probabilistic Detection using Extreme Value Theory (SPADE), which transforms a classifier into an abstaining classifier, offering provable protection against out-of-distribution and adversarial samples. The approach is based on a Generalized Extreme Value (GEV) model of the training distribution in the classifier's latent space, enabling the formal characterization of OOD samples. Interestingly, under mild assumptions, the GEV model also allows for formally characterizing adversarial samples. The abstaining classifier, which rejects samples based on their assessment by the GEV model, provably avoids OOD and adversarial samples. The empirical validation of the approach, conducted on various neural architectures (ResNet, VGG, and Vision Transformer) and medium and large-sized datasets (CIFAR-10, CIFAR-100, and ImageNet), demonstrates its frugality, stability, and efficiency compared to the state of the art.

==> 5_exp_results/fig_eta_delta_data.tex <==

\begin{figure}
    \centering
    \subcaptionbox{\CifarD}{\includegraphics[width=0.24\linewidth]{fig/c10_variation.ps}}    
    \subcaptionbox{\CifarD}{\includegraphics[width=0.24\linewidth]{fig/c10_info.ps}}
    \caption{Test \nOOD\ definition (Definition \ref{def:ood}) against standard OOD datasets. categorized as {\color{blue}{near OOD}} or {\color{orange}{far OOD}} according to \citep{yang2022openood}.}
\end{figure}



==> 5_exp_results/fig_roc.tex <==
 \begin{figure}
    \centering
    \subcaptionbox{\CifarD}{\includegraphics[width=0.3\linewidth]{/fig/ROC_c10.ps}}
    \subcaptionbox{\CifarC}{\includegraphics[width=0.3\linewidth]{fig/ROC_c100.ps}}
    \caption{OOD detection: ROC curve of \XX\ and KNN \citep{pmlr-v162-sun22d} for in-distribution \CifarD\ (Left) and \CifarC\ (Right).}
    \label{fig:roc}
\end{figure}

==> 5_exp_results/tab_ood_SM.tex <==

\begin{table}
    \centering
    \caption{Comparative performance of SPADE (with teacher ResNet) against MSP, ODIN, MDS and KNN:  detection of near OOD, far OOD and adversarial examples on \CifarC\ and \CifarD\ using  AUROC ($\uparrow$) and FPR95 ($\downarrow$) indicators.
    Statistically significantly best performances are in bold.}
    \resizebox{0.75\linewidth}{!}{\begin{tabular}{cccccccc}
    \toprule 
         & & \multicolumn{2}{c}{\textbf{Near OOD}} & \multicolumn{2}{c}{\textbf{Far OOD}} & \multicolumn{2}{c}{\textbf{Adversarial}}  \\
         && \textbf{AUC} $\uparrow$ & \textbf{FPR95} $\downarrow$ &\textbf{AUC} $\uparrow$ & \textbf{FPR95} $\downarrow$ & \textbf{AUC} $\uparrow$ & \textbf{FPR95} $\downarrow$  \\
         \midrule 
         \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\CifarD}}} 
         &MSP \citepalias{hendrycks2018baseline}&87.68&53.54&91.00&31.43&81.96&78.76\\
         &ODIN \citepalias{liang2020enhancing}&80.25&84.49&87.21&60.89&-&-\\
         &MDS \citepalias{lee2018simple}&86.72&46.23&90.20&30.31&81.54&69.14\\
         &KNN \citepalias{pmlr-v162-sun22d} &90.70&\textbf{34.54}&93.11&23.88&85.79&\bf 54.21\\[0.2mm]\cmidrule{2-8} 
         &\bf \XX&\textbf{90.85}&34.74&\textbf{93.44}&\textbf{22.97}&\bf 86.10&54.43\\
         \midrule
         \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\CifarC}}} &MSP \citepalias{hendrycks2018baseline}&80.14&\textbf{55.23}&77.34&59.77&83.46&\bf 50.50\\
         &ODIN \citepalias{liang2020enhancing} &79.86&58.03&78.98&59.34&-&-\\
         &MDS \citepalias{lee2018simple} &58.68&84.22&70.65&72.04&60.27&82.89\\
         &KNN \citepalias{pmlr-v162-sun22d}&80.32&61.33&\textbf{82.64}&53.47&83.72&56.00\\[0.2mm] \cmidrule{2-8}
         &\bf  
\XX&\textbf{80.70}&59.36&81.95&\textbf{53.27}&\bf 84.50&52.72\\
         \bottomrule
         \end{tabular}}
    \label{tab:ood_detection_sm}
\end{table}

